Multiple Contexts and Frequencies Aggregation Network forDeepfake Detection

Deepfake detection faces increasing challenges since the fast growth of generative models in developing massive and diverse Deepfake technologies. Recent advances rely on introducing heuristic features from spatial or frequency domains rather than modeling general forgery features within backbones. To address this issue, we turn to the backbone design with two intuitive priors from spatial and frequency detectors, \textit{i.e.,} learning robust spatial attributes and frequency distributions that are discriminative for real and fake samples. To this end, we propose an efficient network for face forgery detection named MkfaNet, which consists of two core modules. For spatial contexts, we design a Multi-Kernel Aggregator that adaptively selects organ features extracted by multiple convolutions for modeling subtle facial differences between real and fake faces. For the frequency components, we propose a Multi-Frequency Aggregator to process different bands of frequency components by adaptively reweighing high-frequency and low-frequency features. Comprehensive experiments on seven popular deepfake detection benchmarks demonstrate that our proposed MkfaNet variants achieve superior performances in both within-domain and across-domain evaluations with impressive efficiency of parameter usage.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/supp_other_choice_forgery_TS.tex <==
\begin{table*}
  \centering
  \scalebox{0.65}{
  \begin{tabular}{c|c|c|c|c|c|c} \toprule
    \multirow{2}*{Encoder Architecture} & DFD & CDF-v1 & CDF-v2 & DFDCP & DFDC & Avg.\\ 
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-3}
    \cmidrule(lr){4-4}
    \cmidrule(lr){5-5}
    \cmidrule(lr){6-6}
    \cmidrule(lr){7-7}
    & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ & AUC~$\uparrow$ ~\textbar~ AP~$\uparrow$ ~\textbar~ EER~$\downarrow$ \\
    \midrule
    Xception & \textbf{0.888} ~\textbar~ \textbf{0.986} ~\textbar~ 20.3 & 0.823 ~\textbar~ 0.884 ~\textbar~ 23.5 & 0.806 ~\textbar~ 0.882   ~\textbar~ 27.1 & 0.796   ~\textbar~ 0.887 ~\textbar~ 28.5 & 0.729 ~\textbar~ 0.752 ~\textbar~ 34.0 & 0.808 ~\textbar~ 0.878 ~\textbar~ 26.7 \\
    
    EfficientNet-B1 & 0.870 ~\textbar~ 0.983 ~\textbar~ 21.4 & 0.821 ~\textbar~ 0.885 ~\textbar~ 25.1 & 0.809 ~\textbar~ 0.882 ~\textbar~ 27.2 & 0.789 ~\textbar~ 0.881 ~\textbar~ 28.6 & 0.733 ~\textbar~ 0.756 ~\textbar~ 33.5 & 0.804 ~\textbar~ 0.877 ~\textbar~ 27.2 \\

    EfficientNet-B4 & 0.880 ~\textbar~ 0.984 ~\textbar~ \textbf{20.0} & \textbf{0.867} ~\textbar~ \textbf{0.922} ~\textbar~ \textbf{21.9} & 0.830 ~\textbar~ \textbf{0.904} ~\textbar~ \textbf{25.9} & \textbf{0.815} ~\textbar~ \textbf{0.893} ~\textbar~ \textbf{26.9} & 0.736 ~\textbar~ 0.760 ~\textbar~ \textbf{33.0} & \textbf{0.825} ~\textbar~ \textbf{0.893} ~\textbar~ \textbf{25.5} \\
    
    EfficientNet-B5 & 0.877 ~\textbar~ 0.984 ~\textbar~ 21.0 & 0.848 ~\textbar~ 0.919 ~\textbar~ 22.0 & \textbf{0.833} ~\textbar~ 0.898 ~\textbar~ 25.7 & 0.812 ~\textbar~ 0.892 ~\textbar~ 27.1 & \textbf{0.748} ~\textbar~ \textbf{0.772} ~\textbar~ 32.4 & 0.824 ~\textbar~ \textbf{0.893} ~\textbar~ 25.6 \\
    
    \bottomrule
  \end{tabular}
  }
  \caption{
  Performance evaluation of different encoder architectures. All models are trained on the FF++\_c23 dataset and evaluated across various other datasets with metrics presented in the order of AUC~\textbar~AP~\textbar~EER (the frame-level). The average performance (Avg.) across all datasets is also reported. The best results are highlighted in bold.
  }
  \label{tab:other-choice-backbone}
\end{table*}

==> tables/supp_within_entire_synthesis.tex <==
\begin{table}[tb!]
  \centering
%   \vspace{1mm}
  \scalebox{0.75}{
  \begin{tabular}{c|c|c|c|c}
    \toprule
    \multirow{2}*{Method}
    &\multicolumn{4}{c}{Testing Datasets}\\
    \cmidrule(lr){2-5}
    & StarGAN~\cite{choi2018stargan} & DDPM~\cite{ho2020denoising} & DDIM~\cite{song2020denoising} & SD~\cite{rombach2022high} \\
    \midrule
    
    SBI~\cite{shiohara2022detecting} & 0.787 & 0.744 & 0.648 & 0.478 \\

    \midrule

    Ours & \textbf{0.810} &  \textbf{0.854}& \textbf{0.748} & \textbf{0.506} \\
     \bottomrule
  \end{tabular}}
  \caption{
  Results in detecting GAN-generated images and Diffusion-generated images. We compare our results with other augmentation-based SBI~\cite{shiohara2022detecting}. We utilize its official code for evaluation. These models are trained on FF++\_c23. The metric used is the frame-level AUC. ``SD" is the short for stable diffusion.
  }
  \vspace{-10pt}
  \label{tab:ablation_within_entire_synthesis}
\end{table}

